SuperCone: Unified User Segmentation over Heterogeneous Experts via Concept Meta-learning

We study the problem of user segmentation: given a set of users and one or more predefined groups or segments, assign users to their corresponding segments. As an example, for a segment indicating particular interest in a certain area of sports or entertainment, the task will be to predict whether each single user will belong to the segment. However, there may exist numerous long tail prediction tasks that suffer from data availability and may be of heterogeneous nature, which make it hard to capture using single off the shelf model architectures. In this work, we present SuperCone, our unified predicative segments system that addresses the above challenges. It builds on top of a flat concept representation that summarizes each user's heterogeneous digital footprints, and uniformly models each of the prediction task using an approach called "super learning ", that is, combining prediction models with diverse architectures or learning method that are not compatible with each other. Following this, we provide an end to end approach that learns to flexibly attend to best suited heterogeneous experts adaptively, while at the same time incorporating deep representations of the input concepts that augments the above experts. Experiments show that SuperCone significantly outperform state-of-the-art recommendation and ranking algorithms on a wide range of predicative segment tasks and public structured data learning benchmarks.

==> tex/2algorithm.tex <==
\newcommand{\task}{\mathcal{T}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\inp}{\mathbf{x}}
\newcommand{\learner}{f}
\newcommand{\lossi}{\loss_{\task_i}}



\section{Problem Overview}
As illustrated in \autoref{fig-illustration},
our unified system of predictive segments 
will ingest items of interests from a large number of diverse domains such as Hosted Content, Mobile, Advertisement and Finance with
a diverse range of knowledge enrichment, resulting in a heterogeneous information network of users and events, and existing segments.
As a result, the input to our problem is a data-set containing heterogeneous information 
with complex and irregular schema and interconnection.
To address this, we first leverage distributed AutoML technique from \textit{Hadoop-MTA} \cite{li2021automl}
 for data integration and transform 
 each the predictive segment task into an equivalent 
 \textit{unfolded concept learning} task.

Formally, let $\mathcal{S}$ be the set of users (i.e. entity in \cite{li2021automl}) that we predict the segment for
and $\mathcal{Y}$ be the set of possible labels.
 By following \textit{concept unfolding} for ingesting heterogeneous information network,
where different types of interconnections
between entities 
are serialized as an atomic concept
\cite{li2021automl}.
Consequentially, 
we will have a real-valued concept vector 
$(\vec{c_s})$ 
for each user $s$ 
with index being the list of concept vocabulary $\mathcal{C}$ and value being the intensity of its association to corresponding concepts.

For clarity,
we first describe the scenario for 
learning with homogeneous expert.
. Specifically, we assume a particular expert $h_j$, 
associated with a hypothesis space $H_{j} \subseteq \mathbb{R}^{\mathcal{C}} \to \mathcal{Y}$. 
We abstract the  procedure for training the expert and assume an efficient oracle $\theta^{*}_j (\omega; \mathcal{D})$ for obtaining the trained experts
for given dataset $\mathcal{D}$
and 
meta-parameter  $\omega \in \Omega$ for encoding the dependency on the assumptions for "learning to learn", such as model hyper-parameters \cite{franceschi2018bilevel,bayer2009evolving, zoph2016neural, }. 
:
\vspace{-10pt}
\begin{align} \label{eq:metatest}
&
 \theta^{*}_j (\omega; \mathcal{D})
 \defeq \arg\min_{\theta_j \in \Theta_j} R^{\mathcal{D} }_j(h_{j}(\cdot;\theta_j) )  \nonumber\\
& = \sum_{s \in \mathcal{D} }
\mathbf{L}_j(h_j(\vec{c_s}; \theta_j), \mathbf{y}(s)) 
\end{align}
in the hope of minimizing the  generalization error.
Here $\theta_j$ is the set of learn-able parameters contained in the parameter space $\Theta_j$, and $\mathbf{L}_j$ is the loss used for training $h_j$, such as the loss function used for back-propagation. 
% $ \{ \mathcal{D}^{test~(i)}_{target}\}_{i=1}^Q$
The task of unfolded concept learning task
with homogeneous expert can be stated as follows
\begin{Definition} [Unfolded Concept Learning With Homogeneous Expert] \label{def concept}
Assuming the label function of interest
$\mathbf{y}:\mathcal{S} \to \mathcal{Y}$ mapping each user to a label in $\mathcal{Y}$, a probability density of the entity $\mathbf{q} : \mathcal{S} \to [0,1]$, and a sampled dataset $\mathcal{D}$,
the task is to learn a model $\mathbf{h}_j \in H_{j}$,
that minimize the expected risk
according to a given criteria $\mathbf{L}$

\begin{equation*}
\begin{aligned}
& \underset{\omega}{\text{minimize }}
R(h_{j}(\cdot;\cdot,\omega) )
\defeq \mathbb{E}
_{\mathbf{q}}[\mathbf{L}(h_j(\cdot; \theta^{*}_j (\omega; \mathcal{D})), \mathbf{y}(s))]\\
&  = \int_{\mathcal{S}}  
\mathbf{L}(h_j(\vec{c_s}; \theta^{*}_j (\omega; \mathcal{D})), \mathbf{y}(s)
)
\mathbf{q}(s) d s\\
\end{aligned}
\end{equation*}
where $\theta_i \in \Theta_i$ denotes the task specific parameter 
and $\omega \in \Omega$ denotes meta-parameter.  Generalization is then measured by evaluating a number of test points with known labels.
, initialization \cite{finn2017model} or optimizer for $\theta_i$ \cite{bengio1990learning, metz2018meta, schweighofer2003meta}.
\end{Definition}


\begin{figure*}[]
\centering
\includegraphics[width=\textwidth]{fig/SuperconeNN.pdf}
\vspace{10pt}
\caption{Illustration of architecture of \textit{SuperCone}. 
Heterogeneous experts are interconnected and reapplied recursively, where all intermediate outputs are allowed to participate in the final prediction gated by the expert combination network.
An augmentation neural network that learns in parallel to the heterogeneous experts are  learned in the presence to allow sharing and complementing knowledge into the expertise combination stage}
\label{fig-network}
% 
\end{figure*}




\vspace{-10pt}

We start the discussion of unified predictive segments problem
by formalizing the meta-learning problem in  a more general setting.
Consider a distribution over tasks $\mathbf{p}_{\mathbb{T}}: \mathbb{T} \to [0,1]$,
we first assume a source (i.e. meta training) dataset of $M$ tasks sampled from $\mathbb{T}$, 
each containing a training set
(i.e. support set in meta learning literature \cite{bechtle2021meta}) and 
validation set (query set in meta learning literature \cite{bechtle2021meta}) with 
 non-overlapping i.i.d. samples 
 drawn from instances distribution $\mathbf{q}_j$ of task $\mathbf{T}_j$
 , as 
$\mathscr{D}_{source} \defeq \{(\mathcal{D}^{train~(j)}_{source}, \mathcal{D}^{val~(j)}_{source}\}_{j=1}^M$.
Likewise, we assume a target dataset  (i.e. meta test) of $Q$ tasks sampled from $\mathbb{T}$, 
each containing a training set
(i.e. support set in meta learning literature \cite{bechtle2021meta}) and 
validation set (query set in meta learning literature \cite{bechtle2021meta}) with 
 non-overlapping i.i.d. samples 
 drawn from instances distribution $\mathbf{q}_j$ of task $\mathbf{T}_j$
 , as $\mathscr{D}_{target} \defeq \{\mathcal{D}^{train~(j)}_{target}, \mathcal{D}^{test~(j)}_{target}\}_{j=1}^Q$. 
The goal is to obtain the ``meta knowledge'' in the form of $\omega$ from $\mathscr{D}_{source}$ which will then be applied to improve downstream task specific performance in $\mathscr{D}_{target}$,
by adapting and improving based on the individual training set of in the target set in the hope of generalization to the test set.


For the task of learning with heterogeneous experts, however, we are not constrained to the case where source and target set are separate.
Specifically, 
we only require one dataset $\mathcal{D}$ 
to serve as the source dataset, for meta-training, 
and one target dataset, for meta-test.
We assume each of task $j$, $j = 1 \ldots J$, where
the only difference between tasks is the 
particular expert $h_j$, 
each associated with a hypothesis space $H_{j} \subseteq \mathbb{R}^{\mathcal{C}} \to \mathcal{Y}$, a set of learn-able parameter $\theta_j \in \Theta_j$, and a training oracle
$\theta^{*}_j (\omega; \mathcal{D})$ satisfying \autoref{eq:oracle}. The end goal of meta training, then, is to obtain optimal generalization error on the single test target set.  

Formally, we assume
all the available instances will be used for both the source and target set.
 Given a sample of data
$\mathscr{D} \defeq \{\mathcal{D}^{train}, \mathcal{D}^{test}\}$ 
drawn i.i.d from the instance distribution $\mathbf{q}(s)$.
We will use some or all of the instances from $\mathcal{D}^{train}$ for training the individual experts $h_j(\cdot;\theta_j,\omega)$, i.e.
$(\mathcal{D}^{train~(j)}_{source} \subseteq \mathcal{D}^{train},  \mathcal{D}^{val~(j)}_{source} \subseteq \mathcal{D}^{train}$, 
$\mathcal{D}^{train~(j)}_{source} \cap \mathcal{D}^{val~(j)}_{source} = \emptyset $.
Likewise, the dataset used for meta-test consume some or all of the training instances, i.e.,  
$\mathcal{D}^{train~(j)}_{target} \subseteq \mathcal{D}^{train}, j = 1\ldots J$. 
The final goal is to learn a joint model based on the adapted experts on the target training set, 
$\theta^*_j(\omega; (\mathcal{D}^{train~(j)}_{target})$ for $j = 1\ldots J$, denoted as \\
$h(\cdot; \omega, \{h_j(\cdot; \theta^*_j(\omega; \mathcal{D}^{train~(j)}_{target})) \})$,
that achieves the best generalization error. We now have
The unfolded concept learning with heterogeneous experts
can then be defined as joint learning upon $J$ inner training tasks as follows.

\vspace{-10pt}

\begin{Definition} [Unfolded Concept Learning With Heterogeneous Experts]
\label{def concept}
Assuming the label function of interest
$\mathbf{y}:\mathcal{S} \to \mathcal{Y}$, a 
a sampled dataset $\mathscr{D}$, a set of heterogeneous experts $h_j$ with inner training oracle $\theta^*_j(\omega,\mathcal{D})$ for $j = 1\ldots J$,
the task is to learn a combined model $h$ that minimize a given loss criteria $\mathbf{L} : \mathcal{Y} \times \mathcal{Y} \to \mathbb{R}$ 
\begin{align}
& \underset{}{\text{minimize }}
R^{\mathcal{D}^{test}}_{\{H_{j}\}^J_{j=1}, \Omega}
\defeq \nonumber\\
& = R^{\mathcal{D}^{test}}(h(\cdot; \omega^*, \{h_j(\cdot; \theta^*_j(\omega^*; \mathcal{D}^{train~(j)}_{target})) \}) ) \nonumber\\
 & = 
 \sum_{s \in \mathcal{D}^{test} }
\mathbf{L}((h(\vec{c_s}; \omega^*, \{h_j(\cdot; \theta^*_j(\omega^*; \mathcal{D}^{train~(j)}_{target})) \}) , \mathbf{y}(s))
) \label{eq:con-meta}\\
 \text{s.t. } &\omega^* = \arg\min_{\omega} \mathbf{L}^{meta}(
 \{
 \theta^*_j(\omega, \cdot) | j = 1 \ldots J 
 \}, 
 \omega, \mathcal{D}^{train}
 )
\end{align}


\noindent where  ,
$\mathbf{L}^{meta}$ is a meta loss to be specified by the meta-training procedure, such as the cross entropy error of temporal difference error \cite{finn2017model}.
\end{Definition}


The unfolded concept learning with heterogeneous experts abstraction 
extends unfolded concept learningfor efficient and scalable distributed AutoML
and retains the representation power. Using its relation to unfolded concept learning problem  \cite{li2021automl} we have the following results
\begin{Theorem}
The above Unfolded Concept Learning With Heterogeneous Experts problem is no less difficult than
the
Learning In Heterogeneous Data Problem (Definition 1 in \cite{li2021automl}),
Learning In Relational Database (Definition 2 in \cite{li2021automl}),
Heterogeneous Graph Learning (Definition 3 in \cite{li2021automl}), and
First order Logic Graph Learning (Definition 4 in \cite{li2021automl}). 
In fact, there exists efficient linear time reduction from 
Learning In Heterogeneous Data Problem,
Learning In Relational Database,
Heterogeneous Graph Learning, and
First order Logic Graph Learning to Unfolded Concept Learning With Heterogeneous Experts problem.
\end{Theorem}




    \begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{fig/SuperconeTraining.pdf}
    \vspace{10pt}
    \caption{Illustration of the meta optimization procedure. Data-sets for meta-training are recursively constructed by combining the prediction of heterogeneous experts from previous iterations whereas incoming data for meta-test time can be directly applied based on meta-trained models.}
    % \vspace{-10pt}
    \label{fig-optimization}
    \end{figure*}

\vspace{-15pt}
    \section{Choice of $\Omega$}
        
    We divide our discussion of meta learning algorithm into two parts,  the representation of the meta model and the optimization procedure. 
    In this section, we focus on the first part of the meta parameter space $\Omega$ that will be agnostic to the choice of $\Theta_j$ of individual experts $H_j$.
    
    The solution space induced by meta parameter $\omega$ brings inductive bias to the downstream tasks and affect the efficiency of learning procedure of each task. 
    Several key challenges exist for deploying into critical predictive segments systems
    \begin{itemize}
        \item \textbf{Heterogeneous Task Agnosticity} 
        The choice of $\Omega$
        should allow flexibly model a large range of tasks of heterogeneous nature and best utilize the power of experts from $\mathcal{H} = \{H_j | j = 1 \ldots J\}$ depends on the task to be applied, without task-specific engineering.
        \item \textbf{Representation Power} 
        The choice of $\Omega$ should contain enough representation capacity to allow learning deep representation of data  instead of limiting it to specific function class or classification and regression models. 
        \item \textbf{First order influence} 
        The influence of meta parameter $\omega$ should allow for efficient optimization for performance critical application 
         without resorting to higher order gradient estimate \cite{finn2017model} 
        \end{itemize}

    Previous approaches mostly fall into the following categories: traditional super learning and ensemble learning approaches \cite{polley2010super} are heuristic in nature and fail the second criteria;
    traditional deep learning approaches \cite{zhao2019recommending} fail to incorporate the power of experts and fails the first; meta-learning approaches relies on higher order and bi-level optimization \cite{finn2017model} \cite{franceschi2018bilevel}  and are disqualified by the third criteria.
    
    To address this, we present our \textit{SuperAug} architecture that construct a large portfolio of augmented experts and learns deep representation for both direct prediction directly from unfolded concepts and indirect combination of heterogeneous experts, 
    while at the same time respecting their simplicity.
     
    \noindent\textbf{Experts Expansion}
    In the first stage of \textit{Experts Expansion}, 
    we collect possible combinations of experts and construct 
    an augmented set of experts space $\mathcal{H}_{Aug}$ by "cross-breeding" the experts.
    Specifically, the space of  experts $\mathcal{H}_{Aug}$ is constructed such that :
    
    
    \begin{enumerate}
        \item any expert model with hypothesis $H$ belonging to $\mathcal{H}$ will also belong to  $\mathcal{H}_{Aug}$ 
        \item any arithmetic combination between arbitrary number of experts in  $\mathcal{H}_{Aug}$  will also belong to $\mathcal{H}_{Aug}$ 
        \item any recursively application of expert with hypothesis $H$ belonging to  $\mathcal{H}_{Aug}$  over an arbitrary number of outputs from  $\mathcal{H}_{Aug}$ will also belong to $\mathcal{H}_{Aug}$ 
    \end{enumerate}
    The Expert Expansion is implemented in a heterogeneous expert network  in \textit{SuperAug} following a sluice network architecture \cite{ruder2019latent}  along with layer by layer skip connections. As shown in \autoref{fig-network}, the output at each level of densely connected experts $\sigma(\cdot)$ will be fed to both the immediately next level as input as well as to all future levels, and the subsequent connected henceforth.
    
    
    \noindent\textbf{Alternative Experts} 
    In order to augment the model capacity and obtain deep representation of the data, 
    we construct an alternative expert with hypothesis $H_{Alt}$ with a neural network architecture that allow flexible combination of internal components while respect the simplicity of network with lower weights.
    To that end, 
    we follow a neural mixture of experts scheme that captures 
    modularized information across components \cite{jacobs1991adaptive} with an 
    the MMOE architecture\cite{ma2018modeling}.
    Specifically, we divide the neural net into 
    the end output module $\mathbf{Tower}$ that produce the output for the particular task,
    $E$ inner expert neural networks $\mathbf{InnerExpert}_t$, $1\leq t \leq E$, 
    the gating network $\mathbf{Gate}_i$ that project the input into $\mathbb{R}^E$
    from concept vector $\vec{c_s}$.
    The prediction of the final alternative expert that map concept vector $\vec{c_s}$ into label space 
    $\mathcal{Y}$, $h_{alt}(\vec{c_s})$, 
    can be expressed as follows 
    \begin{align}
        h_{alt}(\vec{c_s}) & = \mathbf{Tower}( v_s  ) \\
                v_s &  = \sum_t^{E} \Big( \textrm{softmax} (\mathbf{Gate}(\vec{c_s}))_{(t)} \cdot \mathbf{InnerExpert}_t(\vec{c_s}) \Big) 
    \end{align}    
    where the intermediate representation $v_s$ is a weighted sum by a shallow network $\mathbf{Gate}_i(\vec{c_s^{meta}})$ after normalizing into unit simplex via $\textrm{softmax}(\cdot)$ over inner experts.
    Each $\mathbf{InnerExpert}_t$, in turn, is an ensemble mapping $\vec{c_s}$ to fixed-length vector.Formally, 
        \begin{align}
        \mathbf{InnerExpert}_t(\vec{c_s}) & = \sum_{i=0}^{L} \mathbf{Depth}_{t,i}(\vec{c_s}) \\
                \mathbf{Depth}_{t,i} & = 
        \mathbf{Proj}_{t,i} \Big(\mathbf{Proj}_{t,i-1} 
        \Big(\ldots 
        (\mathbf{Embed}\Big(\vec{c_s}\Big)
        \ldots
        \Big)
        \Big)
    \end{align}   
    where $\mathbf{Depth}_{t,i}$ denotes an intermediate output for the inner expert $t$ at depth $i$, consisting of projection in the form of $\mathbf{Proj}_{t,i}$ which is implemented as a linear layer followed by a non-linear activation.
As illustrated in the alternative expert component in \autoref{fig-network}, an ensemble of neural experts will first be combined to form a deep representation from the concept vector, and further combined with the rest of heterogeneous experts.
        
    
    \noindent\textbf{Combination Network} 
     One distinctive advantage of \textit{SuperAug} over traditional ensemble approaches is the ability to adaptively weight in the different predictions across experts based on the instance. 
    Specifically, assuming the experts from $\mathcal{H}_{Aug}$ are arranged as a array of mappings $\{h_1, h_2, \ldots, h_{\mathcal{H}_{Aug}}\}$,
    the combination network component $\mathbf{Comb}$, will map the concept vector $\vec{c_s}$ into an $|\mathcal{H}_{Aug}| + 1$ dimension vector. We follow the DARTS meta learning \cite{liu2018darts} architecture and produce 
     final model prediction, $h(\vec{c_s})$, as another layer of weighted sums over all possible experts
    \begin{align}
    h ( \vec{c}_s ) = \sum_{t \in \{1, 2,\ldots, T\} \bigcup \{Aug\}} \Big( \textrm{softmax} (\mathbf{Comb}(\vec{c_s}))_{(t)} \cdot h_t(\vec{c_s}) \Big)  \label{eq:final}
    \end{align}
        
    
    \section{meta optimization}
    In this section we describe the approach for optimizing the meta-parameters $\omega$ , agnostic to the heterogeneous experts in $\mathcal{H}$.
    Naive approach that directly treat the original input dataset $\mathscr{D}$ to compute the meta loss $\mathbf{L}^{meta}$ or using it as the support set $(\mathcal{D}^{train~(j)}_{source}$ might lead to "meta-overfit" where the combination network and the added experts in $\mathcal{H}_{Aug}$ falsefully rely on overfitted experts.
    In contrast, we propose a principled framework to construct meta-training set that eliminates the phenomenon and achieves generalization with provable guarantee.
     The high level intuition is to
     extract non-overlapping subset of the data as the support and query set as the source data meta-training to minimize the discrepancy between meta-training and deployment.
     Our optimization method makes no assumption about the heterogeneous experts, including the existence of gradients in its learning process. 
     
     The optimization is shown in \autoref{fig-optimization}, where each level of heterogeneous experts is trained recursively on previous levels with its own meta-training set based on the cross-validation split,
     with the final level corresponding to the \textit{SuperAug} architecture.
     Specifically, we can index heterogeneous experts by the depth it depends on other experts, with $h ^{(k)}_j$ denoting the $j$th expert at $k$th layer, $k = 1, 2,\ldots, K$. 
     At each depth, we have a cross validation scheme, $V^{(k)}$ mapping instance $s$ from $\mathcal{D}^{train}$ to a fold among $1, 2, \ldots, V$, the learning proceed by creating higher-order meta training dataset at each $k$th layer, $\mathcal{D}^{train~(k)}$ as
     \begin{align} 
\mathcal{D}^{train~(k)} & \defeq \{ (\vec{x^{(k)}_s}, \vec{z^{(k)}_s}| 
\vec{x_s} \in \mathcal{D}^{train~(k)}
\} \label{eq:cvtrain1}\\
\vec{z^{(k)}_s}_{(j)} & \defeq 
h ^{(k)}_j(\vec{x_s};\theta^*_j(\omega,(\mathcal{D}^{train~(k-1)})^{ \sim s}) ) \label{eq:cvtrain2}
     \end{align}
with $({D}^{train~(k)})^{ \sim s}$ denoting the subset of $({D}^{train~(k)})$ not in the same fold as instance $i$, formally
\begin{align}
    ({D}^{train~(k)})^{ \sim s} \defeq \{V^{(k)}(s) \neq V^{(k)}(s') | \vec{x_{s'}} \in \mathcal{D}^{train~(k)}\} \label{eq:cvtrain3}
\end{align}
And the meta-parameter $\omega$ is trained using the last layer of the constructed meta-training dataset 
$\mathcal{D}^{train}_{source} \defeq \mathcal{D}^{train~(K)}$, 
with respect to the meta loss defined as follows
    \begin{align}
& \mathbf{L}^{meta}(
 \{
 \theta^*_j(\omega, \cdot) | j = 1 \ldots J 
 \}, 
 \omega, \mathcal{D}^{train}
 ) \defeq   \sum_{\vec{x_s} \in \mathcal{D}^{train}_{source}} \mathbf{L}\Big(h^{train}(\vec{x_s}),
     \mathbf{y}(s) 
 \Big) \label{eq:metaloss}
 \end{align}
 with the meta-training time model $h^{train}(\vec{x_s})$ defined by replacing the output of all heterogeneous experts directly by taking all but the first $|\mathcal{C}|$ elements from the input, $\vec{x_s}_{[:|\mathcal{C}|]}$ and feeding the alternative expert and the combination network with the original feature, $\vec{x_s}_{
     [:|\mathcal{C}|]
     }$. Formally,
 \begin{align*}
    h^{train} ( \vec{x} ) &\defeq \sum_{t \in \{1, 2,\ldots, T\} \bigcup \{Aug\}} v_s^t \\
    v_s^t &\defeq \Big(\textrm{softmax} (
     \mathbf{Comb}(\vec{x_s}_{
     [:|\mathcal{C}|]
     })
     \Big)_{(t)}
      \cdot \Big(
     h_{alt}(\vec{x_s}_{[:|\mathcal{C}|]}), \vec{x_s}_{[|\mathcal{C}|:]}
     \Big)
     _{(t)}
\end{align*}
 The learning of the network parameter thus become and end-to-end optimization problem which can be solved using efficient gradient based methods \cite{liu2018darts}. 
 
 Finally, at meta-test time, the source set for each of the heterogeneous experts $h ^{(k)}_j$, $\mathcal{D}^{train~(k,j)}_{target}$ is defined as the $k$th high order meta training dataset, i.e. $\mathcal{D}^{train~(k,j)}_{target} \defeq  \mathcal{D}^{train~(k)}$
    .
We also have the following results regarding the model's asymptotic and finite sample generalization error over arbitrary heterogeneous expert or the meta learning architecture.

\begin{Theorem}
Assume $\mathcal{Y}$ with bounded cardinality, for any predictive model $\mathbf{y}'$, there exists an parameter space of \textit{SuperAug}  $\Omega$ with the same of less generalization error on instance distribution $\mathbf{q}(s)$  for every instantiation of the data $\mathscr{D}$ in an asymptotic sense. 
Moreover, for float-point based implementation of meta-parameter $\omega$, and $K=1$, then its generalization error will converge to 0 or to the best predictive model under a $O(\frac{log n}{n})$ rate.
\end{Theorem}
\noindent\textbf{Proof} 
We start with the case of asymptotic generalization error.
Consider an arbitrary predictive model $h_1(\cdot)$ with a learning oracle $\theta^*_1( \mathcal{D})$, we construct the following \textit{SuperAug} architecture with a series of heterogeneous experts including $h_1(\cdot)$, 
W.L.O.G. we assume it is the first expert with index 1, since the  \textit{SuperAug} architecture  will further optimize the training time error compared to its input, with probability at least $1 - \delta$ we have
\begin{align}
& \int_{s \in \mathcal{S}}
\mathbf{L}((
h(\vec{c_s}; \omega^*, \{h_j(\cdot; \theta^*_j(
\omega^*; \mathcal{D}^{train~(j)}_{target}
)) \})
, \mathbf{y}(s))
) \mathbf{q}(s) \nonumber\\
\leq & \sum_{s \in \mathcal{D}^{train}_{source} }
\mathbf{L}((h(\vec{c_s}; \omega^*, \{h_j(\cdot; \theta^*_j(\omega^*; \mathcal{D}^{train~(j)}_{target})) \}) , \mathbf{y}(s))
)   + \nonumber\\ & \mathcal{O}
\bigg(
\sqrt{
 \frac{C_1 log |\mathcal{D}^{train}| + C_2 + log 1/\delta}{|\mathcal{D}^{train}|}
)
} 
\bigg) \nonumber\\
\leq & \int_{s \in \mathcal{S}}
\mathbf{L}(h_1(
\cdot; \theta^*_1( \mathcal{D}^{train})
), \mathbf{y}(s))
 \mathbf{q}(s)  + \nonumber\\ &\mathcal{O}
\bigg(
\sqrt{
 \frac{C_1 log |\mathcal{D}^{train}| + C_2 + log 1/\delta}{|\mathcal{D}^{train}|}
)
} 
\bigg)
\nonumber\\
\end{align}

where the first and second in-equality is established with \cite{vapnik1999nature} and $C_1$, $C_2$ are fixed constant. 
For the second part of the theorem, 
again consider an arbitrary predictive model $h_1(\cdot)$, we construct 1 level  \textit{SuperAug} architecture with a series of heterogeneous experts including $h_1(\cdot)$ as the first expert with index 1, along with a series of experts that output the original feature $\vec{x_s}$ into the expert combination $\omega$. If we denote $h^*(\cdot)$ as the expected risk minimizer and $d(h, h^*) \defeq E_{s \sim \mathbf{q}(s)}(
\mathbf{L}(
h(\vec{x_s}), \mathbf{y}(s)
) - 
\mathbf{L}(
h^*(\vec{x_s}), \mathbf{y}(s)
)
)$ be the expected performance of a model $h$,
by leveraging 
the 
 results in Equation 2 in \cite{van2007super},
  from which the convergence results will follow from the fact that 
  for every $\delta > 0$ there exists a constant $C$ that 
\begin{align}
    & \frac{1}{V} \sum_{v=1}^V E d(h(\vec{c_s}; \omega^*, \{h_j(\cdot; \theta^*_j(
\omega^*; \{\vec{x_s} \in \mathcal{D}^{train}, V^{(0)}(s) = v\}
)) \}), h^*) \nonumber\\
\leq & (1+\delta) E \min_{\omega \in \Omega} \frac{1}{V}  \sum_{v=1}^V  d(h(\vec{c_s}; \omega, \{h_j(\cdot; \theta^*_j(
\omega; \nonumber
\{\vec{x_s} \in \mathcal{D}^{train}, V^{(0)}(s) = v\} \nonumber\\ &
)) \}), h^*) 
+ C \frac{V log |\mathcal{D}^{train}|}{|\mathcal{D}^{train}|}
\end{align}
\vspace{-10pt}

==> tex/3exp.tex <==
\newcommand{\madelon}{\texttt{madelon}}
\newcommand{\ana}{\texttt{a9a}}

\input{sub_tex/table/app}


\begin{figure*}[]
\centering
% \vspace{-10pt}
\includegraphics[width=.9\textwidth]{fig/Superconcore.pdf}
% \vspace{-10pt}
\caption{Performance comparisons of weighted one-versus-result ROC-AUC, weighted F-1 Score, Log loss across the 39 different types of predictive segment tasks}
\label{fig-AUC}
\end{figure*}
 

\begin{figure*}[]
\centering
% \vspace{-10pt}
\includegraphics[width=\textwidth]{fig/Superconecorecost.pdf}
\caption{Model cost measured in microseconds over the 39 production predictive segment tasks}
\label{fig-inference cost}
% \vspace{-10pt}
\end{figure*}






\begin{figure}[]
\centering
\includegraphics[width=.5\textwidth]{fig/Superconablation.pdf}
\caption{
Distribution of change in model performance and model cost across \textit{SuperCone} variants.
}
\label{fig-qualitative}
\vspace{-10pt}
\end{figure}

\begin{figure}[]
\centering
\includegraphics[width=.5\textwidth]{fig/Superconeinterpretability}
\caption{Experts attention learned by \textit{SuperCone} averages across datasets}
\label{fig-Interpret-ability study on task relation learning}
\vspace{-10pt}
\end{figure}


\section{EXPERIMENT}
In this section, we present a series of experiments centered around the following research questions: 
\begin{itemize}[leftmargin=2.5em]
    \item[\bf RQ1] How do  alternative methods compare to SuperCone according to core performance metrics used for production?
    \item[\bf RQ2] How do the settings and individual components of SuperCone affect its quality? 
    \item[\bf RQ3] How does the approach of SuperCone compares with other methods when applied to public structured data learning tasks?
    \item[\bf RQ4] Is the approach of SuperCone reliable when applied to different tasks of different types  and domains and interpretable to human inspection?
    \item[\bf RQ5] How does SuperCone perform under resource constrained scenario and balance between the performance and computation cost?
    \item[\bf RQ6] How does SuperCone compared against alternatives in production environment for key end goals? 
    
\end{itemize}

\noindent\textbf{Data-set}
We used both proprietary and public datasets. 
For the former, we collected and compiles a total of 39 different predictive segment tasks involving discretized range prediction, multi-class classification prediction as well as binary classification prediction from production.
It is constructed by associating
users with interest taxonomy including 
YCT, OIC \cite{zhou2016predicting}, 
 as well as open-domain knowledge base including Wikipedia and Price-Grabber. 
 The dataset contains 100K dimensional unfolded vector per instance, with a total of 100K instances. 
 Each of the 39 dataset is split into 3 folds, with 2/3 of them belonging to the support set and remainder belonging to the hold-out query/test set.
 
We also compare our approaches over several public benchmark dataset.
Specifically, we use the 
 \madelon \cite{guyon2004result} 
 and 
 \ana \cite{platt1998sequential}.
 \madelon contains 2,000 training samples, 600 test samples with 500 features per sample. \ana contains 32,561 training samples, 16,281 test samples with 123 features per sample, respectively.
 		
 

\noindent\textbf{Methods Comparison}
We implement \textit{SuperCone} in two variants.
The first variant is a homogeneous neural network version that predicts the outcome with purely the neural alternative expert $H_{Alt}$ and the expert combination architecture following a multi-gated neural mixture of expert (\textit{MMOE}) \cite{zhao2019recommending} architecture,
where each one is by itself constructed recursively with an \textit{MMOE},
with the inner MMOE for $H_{Alt}$ having 3 experts 3 layer of densely connected residual connection as shown in Equation 7 with a width of 32, and gate network having 2 layer of densely connected residual connection shown in Equation 7 with width 32,
and the inner MMOE for the combination network having 3 layer of densely connected residual connection as shown in Equation 7 with a width of 32. We denote this the \textit{Multi-MMOE}.
We then use the exact same network architecture and combine it with heterogeneous expert set with $|\mathcal{H}_{Sug}| = 70$ and $K=2$  for public benchmark and the production supported $|\mathcal{H}_{Sug}| = 31$ and $K=1$ experts for the proprietary datasets,
including 11 hyperparameter-tuned gradient boosting models under various implementation trained on GPU accelerators.
The learning rate is tuned using an exponent search and set as 1e-4 with epoch of 30.
The setting is applied to all datasets.

In addition, we implement the following baseline approaches


\begin{itemize}


\item \textbf{PLE} implements the Progressive Layered Extraction method \cite{tang2020progressive} using shared expert count as 1 and  specific expert as 2 , with expert layer width as 256, 256, gate layer width as 16, 16, and tower layer depth as 32, 32.
\item  \textbf{WDL} implements wide and deep learning  \cite{cheng2016wide} with the deep network  layer width tuned as 8 for \madelon and 256, 128, 64 tuned for the rest datasets.
\item  \textbf{ESSM}  implements Entire Space Multi-Task Model \cite{ma2018entire} with CTR component and CVR component each with 
layer width as 512, 512.
\item  \textbf{DCN} implements Deep \& Cross Network \cite{wang2017deep} with layer width as 384, 128, 64, cross count as 2 and cross dimension as 100.
\item  \textbf{DCNMix}  implements Cost-Effective Mixture of Low-Rank DCN \cite{wang2021dcn} with  per layer experts count as 4 and width as 256, 128, 64, cross count as 2 and cross dimension as 100 with a rank of 32.
\end{itemize}
All online adaptation and single task learning was performed with 30 epochs of Adam optimization with a tuned learning rate between 1e-6 and 1e-5 depends on the dataset. The rest settings default to the implementation reported in the  original paper.

\noindent\textbf{Core Performance Evaluation [RQ1, RQ4] }
First and foremost, 
we compare the performance of various candidate approaches 
over the 39 production predictive segment tasks,
and score their performance using the weighted 
one-versus-all ROC-AUC (Weighted OVR AUC) that applies to range-prediction, multi-class prediction and binary prediction,
as well as the weighted F1 score and cross-entropy log loss that also applies to the different 
types of prediction tasks simultaneously.
As shown in \autoref{fig-AUC}, 
\textit{SuperCone} that is implemented agnostic to tasks does not suffer from 
overfitting or meta-overfitting, and is able to consistently outperform benchmarks and achieves close to 100 \% F1-score and ROC-AUC without tuning.
With other strong baselines including \textit{Multi MMOE}, \textit{PLE} and \textit{ESSM}.

\noindent\textbf{Public Benchmark Evaluation  [RQ3,RQ4]}
We further evaluate the applicability of \textit{SuperCone} on public structured dataset aganist the best performing version of baselines, where 
the Multi MMOE methods degrades to MMOE architecture \cite{zhao2018deep}.
Table 1 reports the absolute value of various performance metrics 
including Accuracy, ROC-AUC (AUC), Cohen-Kappa Score (Kappa), F1 Score (F1) and Log loss,
as well as its relevant change compared to baseline \textit{WDL} of 
and the aggregated the overall change across metrics.
Again, \textit{SuperCone} without task specific tuning is able to achieve consistent performance, improving on competitive baseline by a significant margin.

\noindent\textbf{Computation Cost [RQ5] }
We then study the computation cost of various approaches that are of critical important for
cost and latency sensitive production system.
Specifically, we measure the computational cost in a per distributed-executor node setting, 
where shard-ed dataset are sent to local node and processed sequentially.
\autoref{fig-inference cost} shows the number of microsecond to process a single data instance, where
 \textit{SuperCone} requires similar cost because heterogeneous expert outputs only amounts to small portion of the feature sets,
 and thus achieving a better tradeoff point between performance and cost. 

\noindent\textbf{ Ablation Analysis [RQ2]}
We investigate the impact of meta training over heterogeneous experts (see Algorithm 1) by comparing the distribution of 
performance gain and cost change in terms of Weighted OVR ROC-AUC over 
from \textit{SuperCone} and its ablation version without heterogeneous experts, i.e. the \textit{Multi MMOE} approach.
The left figure of \autoref{fig-qualitative} shows the distribution of relative gain in performance
while the right figure of \autoref{fig-qualitative} shows the distribution of relative cost, aggregated over the 39 production predictive segment tasks.
We can observe that \textit{SuperCone} 
achieve a significant improvement over the already competitive 
ablation version with cost  distributed closely around zero in a highly symmetric fashion.


\noindent\textbf{Interpret-ability Study [RQ2,RQ3]}
We next investigate the interpret-ability of \textit{SuperCone} 
by visualizing the meta-learned expert attention average across instances and datasets
for the domain of proprietary predictive segments tasks,
\madelon, and \ana.
Specifically, for each dataset, 
we extract the instantiated combination network output $\textrm{softmax} (\mathbf{Comb}(\vec{c_s}))_{(t)}$ as shown in Equation 8, 
for the $|\mathcal{H}_{Aug}| + 1$ experts, with neural alternative methods followed by the heterogeneous experts.
As shown in \autoref{fig-Interpret-ability study on task relation learning}, 
expert attention displays an even distribution across the multiple experts,
with the proprietary domain more biased towards models  with GPU accelerator and scale to dataset with much larger instances count and more features. 

\begin{table}
\vspace{-10px}

\label{tab:age segment}
\setlength\tabcolsep{1pt} % default value: 6pt

\resizebox{.5\textwidth}{!}{% <------ Don't forget this %
\centering
\begin{tabular}{c|c|c|c|c|c}
\rowcolor[HTML]{C0C0C0}
\textbf{} & \textbf{Accuracy} & \textbf{Recall} & \textbf{Precision} & \textbf{Weighted F1} & \textbf{Cohen Kappa} \\ \hline
Previous Production & 0.20   & 0.23  & 0.28          & 0.21   & 0.08   \\ \hline
SuperCone          & 0.42   & 0.42 & 0.42 & 0.41   & 0.27   \\ \hline
Lift                & +112.54\% & +78.47\% & +47.39\%         & +89.85\% & +249.61\%
\end{tabular}

}

\caption{Comparison of \textit{SuperCone} with the previous production system on range prediction use cases}
% \vspace{-10px}
\end{table}
\noindent\textbf{Online evaluation [RQ6,RQ4]}
The \textit{SuperCone} is rolled out to production targeting use cases 
in internal Hadoop based deployment system and evaluation in key range predication tasks
Table 2 shows the performance comparison between \textit{SuperCone} and previous production system, which shows that 
the meta-training paradigm generalizes well to the new incoming data and compares favorably in the practical setting.


==> tex/9conclusion.tex <==
\section{Conclusion}

In this work, we present \textit{SuperCone} as our  solution for predicative segments system that is able to handle 
task heterogeneity, 
data scarcity and 
long tailness, by integrating heterogeneous experts and combining them in the end to end fashion, following a principled meta-learning approach.
Extensive evaluation on large number of predicative segments tasks and public benchmarks datasets demonstrate the reliability and superior performance of  \textit{SuperCone} over state of the art recommendation and ranking approaches in key production use cases.

One particular interesting directions for future research is to extend the \textit{SuperCone} paradigm for wider range modality and domain and more applications tasks for social good, another is to build more universal representation and better integration with common knowledge base towards commonsense AI.
